Trustworthy Refactoring via Decomposition and Schemes: A Complex Case Study

Widely used complex code refactoring tools lack a solid reasoning about the correctness of the transformations they implement, whilst interest in proven correct refactoring is ever increasing as only formal verification can provide true confidence in applying tool-automated refactoring to industrial-scale code. By using our strategic rewriting based refactoring specification language, we present the decomposition of a complex transformation into smaller steps that can be expressed as instances of refactoring schemes, then we demonstrate the semi-automatic formal verification of the components based on a theoretical understanding of the semantics of the programming language. The extensible and verifiable refactoring definitions can be executed in our interpreter built on top of a static analyser framework.

==> eptcsdata.tex <==
\providecommand{\firstpage}{92}
\providecommand{\publicationstatus}{A. Lisitsa, A. Nemytykh, M. Proietti (Eds.): \\
Verification and Program Transformation (VPT 2017)\\
EPTCS 253, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.253.8}{10.4204/EPTCS.253.8}}
\pdfoutput=1

